Knowledge-Based Version Incompatibility Detection for Deep Learning

Version incompatibility issues are rampant when reusing or reproducing deep learning models and applications. Existing techniques are limited to library dependency specifications declared in PyPI. Therefore, these techniques cannot detect version issues due to undocumented version constraints or issues involving hardware drivers or OS. To address this challenge, we propose to leverage the abundant discussions of DL version issues from Stack Overflow to facilitate version incompatibility detection. We reformulate the problem of knowledge extraction as a Question-Answering (QA) problem and use a pre-trained QA model to extract version compatibility knowledge from online discussions. The extracted knowledge is further consolidated into a weighted knowledge graph to detect potential version incompatibilities when reusing a DL project. Our evaluation results show that (1) our approach can accurately extract version knowledge with 84% accuracy, and (2) our approach can accurately identify 65% of known version issues in 10 popular DL projects with a high precision (92%), while two state-of-the-art approaches can only detect 29% and 6% of these issues with 33% and 17% precision respectively.

==> pre-knowledgeextraction.tex <==
We structure the extracted data into a probability knowledge graph which can portray relations between software libraries, APIs, frameworks, and hardware devices ~\cite{cummaudo2020interpreting}.

\subsection{Problem Formulation}
We extract the logic facts from Stack Overflow where developers worldwide share their knowledge on software, library and hardware related problems. To extract knowledge from Stack Overflow, we obtain a huge set of Stack Overflow posts related to Deep Learning and then pass it on to a relevancy checker to filter the posts which contains version and entity information. The relevancy checker takes in sentences from a post as input and selects the posts satisfying the constraints. The remaining posts are discarded by the relevancy checker. 

The relevant posts are then passed to the version extraction component which extracts the versions from the sentence. Our Entity extractor component parallelly filters the named entities from the sentence. The extracted entities and the versions data are then passed to the version entity matcher component which associates the entities to its version based on parsing tree mechanism. The version entity pairs are then passed to a pretrained Unified QA Model which predicts the relationships between two different entities based on the sentences. The compatibility relationships are then clustered into a knowledge base and then passed to the compatibility detection part.
\begin{algorithm}
\caption{Knowledge Base Creation Heuristic}\label{algorithm}
\KwIn{$ S = \{Posts\}$}
\KwOut{$K$ = \{CK, ICK\}}

\BlankLine

$K \leftarrow \{\} $; \ $CK \leftarrow \{\} $ ; \ $ICK \leftarrow \{\} $

\ForEach{$s$ in $S$}{
$ relevant_{s} \leftarrow checkVersionEntityInfo(s) $;

\eIf{$relevant_{s} == true$}{
$ v_{s} \leftarrow extractVersionInfo(s) $ \;
$ e_{s} \leftarrow extractEntityInfo(s) $ \;
$res \leftarrow  \{v,e,c/ic\}$  
$res \leftarrow matchVersionEntity(v_{s}, e_{s})$ \;
\eIf{c in res}{
$CK.add(res)$\;
}
{
$ICK.add(res)$\;
}
}
{
$continue$;
}
}
return K
\end{algorithm}

\subsection{Data Collection}

\subsubsection{Data ffff}
Figure x shows the architectural diagram of our approach. Our dataset comprises over 50k posts from stackoverflow tagged with [Tensorflow]. The parsing of StackOverflow posts is done through XML parsing and the posts are stored in XML format. Each question post contains information such as the \textit{Post Id, PostTypeId, AcceptedAnswerId, ParentId	CreationDate, DeletionDate, Score, ViewCount, Body, OwnerUserId, Title} and \textit{Tags}. For each question post, we perform another scraping process is performed where the answer posts with PostTypeId = 2 are obtained by matching against their questions. The answer scraping process is done because the logic facts we are interested in would be present in the answer posts. 

We have obtained over 50k answer posts with the help of the above method. To check whether a sentence focuses on version compatibility, we have developed a relevancy checker which filters the relevant sentences focusing on version compatibility. The relevancy checker makes use of POS tagging to filter the named entities and regex pattern matching for obtaining the version information (Explained more in section 3.3). If the frequency of named entities is greater than 1 and if there is a version number present, then the sentence is considered relevant.

In this way, the relevant sentences are filtered. The input dataset comprising of over 10k relevant posts have been obtained from the questions posts and they are now passed to the knowledge extraction module where the versions, entities are extracted and matched against each other.  

\subsection{Named Entity Recognition}

\noindent{\bf Version Extraction}
After obtaining the SO sentences, the next step involves Version Extraction involving extraction of the version numbers of different libraries present in the posts, e.g. v2.0, version 3.8.  The regex pattern along with an example is shown in Figure x. 

\includegraphics[scale = 0.5]{Screen Shot 2022-04-20 at 2.12.18 PM.png} \\
All the version numbers represented in different forms are extracted and gathered into a list. This list is then passed to the version entity matcher.

\noindent{\bf Entity Extraction}
We also extract the named entities in sentences to filter out the software engineering terms. To filter the named entities for the sentences, we have devised a new approach to filter the software engineering terms from a sentence. The new approach involves the data collection of the tags from Stackoverflow posts relevant to deep learning and then comparing the tags against the named entities in a sentence. If the named entity is associated with a tag relevant to deep learning, then the named entity is extracted. This way we have made use of a technique to extract the software engineering terms from a sentence. Our approach performs better than the state of the art approaches in this space. The following is the figure comparing our approach against Wikifier and Domain Thesaurus.

\noindent{\bf Version Entity Matcher}
Once we have obtained the version and entity information, we perform the Version Entity Matching to match the extracted version number with the corresponding library or framework intended in the post. This component in the pipeline makes use of a parse tree to compute the distance between an entity and a version. This works by mapping a sentence to a Context Free Grammar in the form of a constituency parsing tree. The Version Entity Matcher's information are then passed on to a pretrained Question Answering model.  When presented with the sentence and a compatibility question, the pretrained QA model generates a Yes/ No answer. To make sure the results of the QA model are accurate, we make use of a loss metric associated with each prediction and compute the loss. Based on a preset threshold value, we determine the correctness of a prediction. If the loss value is less than the threshold, then the model is confident with the prediction and hence this prediction result is used to generate the logic facts.  

\subsection{Relation Extraction via Question Answering}

\todo{Yimaz needs to write about this.}
Explain about Yes or No questions. Talk about the novelty.

\subsection{Knowledge Consolidation}

\todo{Zhongkai needs to write about this.}

